MutaPLM: Protein Language Modeling for Mutation Explanation and Engineering

Studying protein mutations within amino acid sequences holds tremendous significance in life sciences. Protein language models (PLMs) have demonstrated strong capabilities in broad biological applications. However, due to architectural design and lack of supervision, PLMs model mutations implicitly with evolutionary plausibility, which is not satisfactory to serve as explainable and engineerable tools in real-world studies. To address these issues, we present MutaPLM, a unified framework for interpreting and navigating protein mutations with protein language models. MutaPLM introduces a protein delta network that captures explicit protein mutation representations within a unified feature space, and a transfer learning pipeline with a chain-of-thought (CoT) strategy to harvest protein mutation knowledge from biomedical texts. We also construct MutaDescribe, the first large-scale protein mutation dataset with rich textual annotations, which provides cross-modal supervision signals. Through comprehensive experiments, we demonstrate that MutaPLM excels at providing human-understandable explanations for mutational effects and prioritizing novel mutations with desirable properties. Our code, model, and data are open-sourced at https://github.com/PharMolix/MutaPLM.

==> 1_introduction_old.tex <==
\section{Introduction}
% Introduction to protein representation learning and mutation understanding. However, their application is compromised due to misalignment with human preferences.
Understanding protein evolution through mutations in amino acid sequences serves as the mainstay in life sciences for elucidating biological diversity \cite{}, informing biotechnological applications \cite{}, and developing novel therapeutic agents \cite{}. Recently, deep learning approaches \cite{} have been proposed to comprehend protein sequences, culminating in the emergence of protein language models (PLMs) like ESM \cite{}. Pre-trained on evolutionary-scale protein databases \cite{}, PLMs have shown great promise in predicting protein structure \cite{}, protein function \cite{}, and mutational effects \cite{}. 

% Advances in protein-text LLMs.
Despite their promising advancements, existing black-box PLMs fall short in providing specific explanations or customized navigation for protein evolution. To this end, recent works that bridge protein sequences and biomedical texts with large language models (LLMs) \cite{} have emerged. One line of works \cite{} attempts to jointly incorporate proteins and texts within a unified model. Another line \cite{} connects PLMs with large language models (LLMs) \cite{} through instruction tuning \cite{}. These studies have shed light on LLMs' intelligence and versatility in revolutionizing protein-related research applications.

%  %For example, BioMedGPT \cite{} aligns ESM-2 \cite{} and LLaMA-2 \cite{} with a linear adaptor and performs fine-tuning on a question-answering dataset for proteins. Mol-Instructions \cite{} proposes to enhance LLMs' comprehension of the protein sequences with instruction-tuning.

% InstructProtein \cite{} collects protein instruction-tuning data from a knowledge graph. ProtLLM \cite{} proposes to model proteins as words that interleave with text tokens. 

% Challenges: (1) Aligning the global and local landscape of proteins. (2) Mitigating catastrophic forgetting.
Motivated by the success of connecting PLMs and LLMs, we aim to interpret and design protein mutations with natural language, a research arena that is under-explored due to the following challenges: (1) First, directed evolution \cite{} involves proposing a small number of mutations. Unfortunately, existing strategies for text-based protein sequence design are mostly developed for de-novo generation \cite{}. (2) More importantly, modeling mutations requires a holistic understanding of both the local protein fitness landscape \cite{} and the global protein property landscape. However, prior works primarily focus on global protein properties rather than local fitness, where subtle changes in amino acids may drastically alter protein functions. 

% (2) Secondly, fine-tuning PLMs and LLMs on sparse mutation data may lead to catastrophic forgetting of the original protein and textual knowledge, a phenomenon known as 'alignment tax' \cite{}. 

% Solution: (1) bi-directional architecture (2) two-stage pre-training + CoT
In this work, we propose e-ESM, an ESM copilot for text-based protein evolution explanation and design, to address the aforementioned issues. We present a brief illustration in Figure. \ref{}. In addition to transforming protein sequences into soft tokens for LLM explanations, we propose a bi-directional fusion architecture that allows the PLM to integrate textual information from the LLM and propose novel mutations. To jointly harness local and global protein landscapes, we develop a two-stage training paradigm. The first pre-training stage aligns the PLM and LLM with extensive protein-related literature. The second fine-tuning stage allows our model to infer mutational effects or design mutations based on protein function information in a Chain-of-Thought (CoT) \cite{} manner.

Additionally, we present MutDescribe, a large-scale dataset with single-site mutations and textual descriptions of mutational effects. MutDescribe is collected by expert annotations from structured databases, ChatGPT \cite{} annotations from unstructured sources, and ESM \cite{} annotations involving first-principle protein knowledge. Thanks to this dataset, we improve our model's proficiency in grasping protein evolution.

% Experiments
We perform comprehensive experiments on two novel tasks that bear promising application significance: mutation explanation and text-based mutation design. Plentiful evaluations and case studies show that e-ESM significantly outperforms existing protein-text models and GPT-4 in accuracy and factuality. Additionally, e-ESM bridges PLM with real-world directed evolution by prioritizing mutants that satisfy free-text prompts and exhibit high fitness scores. 

% Conclusions
Our contributions are summarized as three folds:

\begin{itemize}
\item We present e-ESM, an ESM copilot built upon a large language model. With a bi-directional architecture and two-stage training, e-ESM can jointly harness the local and global protein landscapes and facilitate text-based protein evolution explanation and design.
\item We introduce MutDescribe, a large-scale protein mutation dataset. To the best of our knowledge, it is the first dataset that involves textual annotations for protein mutations.
\item Through comprehensive experiments, we demonstrate the superiority of e-ESM in explaining mutational effects and proposing high-fitness mutations based on textual instructions.
\end{itemize}
